Understanding disentangling in $\beta$-VAE

We present new intuitions and theoretical assessments of the emergence of disentangled representation in variational autoencoders. Taking a rate-distortion theory perspective, we show the circumstances under which representations aligned with the underlying generative factors of variation of data emerge when optimising the modified ELBO bound in $\beta$-VAE, as training progresses. From these insights, we propose a modification to the training regime of $\beta$-VAE, that progressively increases the information capacity of the latent code during training. This modification facilitates the robust learning of disentangled representations in $\beta$-VAE, without the previous trade-off in reconstruction accuracy.

==> acknowledgements.tex <==
\section*{Acknowledgements}
\label{S:acknowledgements}


==> notes.tex <==

_________________________________

This is Sec.\ \ref{S:intro}. This is an equation:

\begin{align} \label{E:concept}
    C_i = \{ (k, p_k^i(Z_k)) ~|~ k \in S_{i}  \}
\end{align}

where $S_{i} \subseteq \{1, ..., K\}$ is stuff in Eq.\ \ref{E:concept}. There is also a Fig.\ \ref{F:figure}.

\begin{figure}[ht]
 \centering
 \includegraphics[width = 0.3\textwidth]{figures/temp.png}
 \vspace{-6pt}
 \caption{An example figure} 
 \label{F:figure}
\end{figure}
----
following insights from disentangling in bvae, we propose a disentangled representational space as one which arranges the datapoints onto a compact set of axes where nearby points are also close in dataspace, and where those axes correspond to qualitatively different features of variation in the data. we propose that those features can be discriminated by the differing contribution that information about them makes to reconstruction accuracy.
----
we want the equations for the latent distribution, noting the reparam, and equations for the simplified form of the KL with the unit gaussian
----

--- what follows is some misc notes to be removed later ---
Here the pressure may be too weak to fully regularise the representation in this way. At the boundaries between clusters, there could be representational discontinuities. In the context of stochastic gradient descent, as the datapoints are arranged in latent space initially somewhat randomly early in training, a weak KL/bottleneck pressure would only be enough to encourage weak/localised overlap in general. this could leave discrete clusters where the datapoints are well ordered within them, but arranged out of order globally, (i.e. with representational discontinuities as you cross from one to the other - a smooth traversal in latent space jumps to a relatively distant datapoint). The weak pressure (i.e. cost for the discontinuties) and their clustering means the optimization would have have trouble rearranging ``disentangling'') these clusters. 

latent/representational embedding of data points continuously along the data manifold
At this point, at least two reasons to encode this new factor into a distinct latent dimension:
 - another locality-preserving axis allowing maximal overlap
 - different contribution to reconstruction: can assign appropriate precisions to the scale and x/y latent dimensions
 
 (todo: point out somewhere that x and y are aligned due to their uniform distribution)
 
 --- finds components in the data which make different contributions to reconstruction, and sorts them into different latent dimensions, *since the model will be able to assign them each a different encoding capacity/precision optimal for their contribution*.

stable point of optimization when $dLL/dKL = \beta$, i.e. all else being constant, beta sets the ratio of the trade-off: the smallest pay off in log likelihood gain per unit KL that the optimization will maintain
---
mention
 - symmetry of x/y position versus most other factors lacking symmetry
---

for version 2:
 - show samples from the prior are better and discuss why
 - super-toy 2d dataset with different reconstruction contributions by construction
 showing if we construct components with different reconstruction contributions, the latent code ends up axis-aligned to them, otherwise it's just a random rotation of them
 - correlations in the data. held out central positions, still generalise well. simple correlations in the toy 2d dataset
 - disentangling metric based on representation with "factorised" decoder likelihood. measure the off diagonal hessians



